Protecting Facial Privacy: Generating Adversarial Identity Masks via Style-robust Makeup Transfer

While deep face recognition (FR) systems have shown amazing performance in identification and verification, they also arouse privacy concerns for their excessive surveillance on users, especially for public face images widely spread on social networks. Recently, some studies adopt adversarial examples to protect photos from being identified by unauthorized face recognition systems. However, existing methods of generating adversarial face images suffer from many limitations, such as awkward visual, white-box setting, weak transferability, making them difficult to be applied to protect face privacy in reality. In this paper, we propose adversarial makeup transfer GAN (AMT-GAN), a novel face protection method aiming at constructing adversarial face images that preserve stronger black-box transferability and better visual quality simultaneously. AMT-GAN leverages generative adversarial networks (GAN) to synthesize adversarial face images with makeup transferred from reference images. In particular, we introduce a new regularization module along with a joint training strategy to reconcile the conflicts between the adversarial noises and the cycle consistence loss in makeup transfer, achieving a desirable balance between the attack strength and visual changes. Extensive experiments verify that compared with state of the arts, AMT-GAN can not only preserve a comfortable visual quality, but also achieve a higher attack success rate over commercial FR APIs, including Face++, Aliyun, and Microsoft.

==> section/3-method.tex <==
\section{Adversarial Makeup Transfer GAN (AMT-GAN)}\label{method}
\subsection{Problem Formulation}
In this section, we first formulate the goal of adversarial attack on deep face recognition models (or protect image privacy against deep face recognition models in other words). Then we will combine them with the make-up transfer problem.

Adversarial attack on face recognition system can be summarized as:
\begin{equation}\label{eq:adversarial fomulation}
\begin{aligned}
    % \left\{L_{adv} = D(M_l(x^C),M_l(x^A)) \right\}
      \left\{ \begin{aligned}
        &\max \limits_{x^A} L_{adv} = D(M_k(x^C),M_k(x^A)) \text{for dodging,}\\
        &\min \limits_{x^A} L_{adv} = D(M_k(x^A),M_k(z))\text{for impersonation,}
       \end{aligned}
 \right.
\end{aligned}
\end{equation}
where the $D(\cdot)$ represents a distance function such as cross entropy or cosine similarity, and $M_k$ represents a DNN-based feature extractor for face recognition. $x^C$, $x^A$, and $z$ stand for the original image, adversarial example, and target image respectively. In dodging attacks, adversaries want to change $x^C$ to $x^A$ which can be recognized as someone else by face recognition models, while in impersonation attacks, the $x^A$ is supposed to be recognized as the specific identity as same as $z$.

In this paper, we combine the adversarial attacks with make-up transfer technique. Let \textit{$X \subset \mathbb{R}^{H \times W \times 3}$} and \textit{$Y \subset \mathbb{R}^{H \times W \times 3}$} be the source make-up style and the reference make-up style domain. Here, we use \textit{$\{x^C_n\}_{n=1,...,N }$},\textit{$x^C_n \in X$} and \textit{$\{y^C_m\}_{m=1,...,M }$},\textit{$y^C_m \in Y$} to represent the clean face images with the source make-up style and the reference make-up style respectively, \textit{$\{x^A_n\}_{n=1,...,N }$},\textit{$x^A_n \in X$} and \textit{$\{y^A_m\}_{m=1,...,M }$},\textit{$y^A_m \in Y$} to represent the adversarial face images with the source make-up style and the reference make-up style respectively, where \textit{$n, m$} represent the identity information. The goal of the adversarial make-up transfer is to train a function \textit{$G$}: \textit{$\{x^C_n, y^C_m\} \to \tilde{y}^A_n$},  where the generated image \textit{$\tilde{y}^A_n$} has the same make-up style compared to the reference image \textit{$y^C_m$}, preserves the visual identity from the source image \textit{$x^C_n$}, and can be used to lunch dodging attack or impersonation attack to deep FR models.

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{figures/figure_pipe.pdf}
\caption{The architecture of the proposed TBD-GAN.}
\label{fig:pipe}
\end{figure*}

\subsection{Framework}
\textbf{Overall.} The architecture of the proposed TBD-GAN is depicted in Fig~\ref{fig:pipe}.

\textbf{Generator \textit{$G$} and Discriminators $D_X,D_Y$.} Generative adversarial networks~\cite{DBLP:journals/corr/GoodfellowPMXWOCB14} are widely used and proven to have outstanding performance in image-to-image translation tasks such as style transfer, restoration, image segmentation, and pose estimation. Recently studies~\cite{DBLP:conf/mm/LiQDLYZL18,DBLP:conf/cvpr/JiangLG0HFY20} show that GANs are also very competitive for make-up transfer which can be regarded as a variety of style transfer. Therefore, in our proposed framework, we consider a group of generative adversarial networks as our main networks, including a generator and a pair of discriminators. The generator $G$ is supposed to turn the style of source images from the source domain into reference domain and add adversarial modification on them. The discriminators $D_X$ and $D_Y$ are supposed to distinguish the fake images generate by $G$ from the real natural distribution. Specifically, in the training process, $D_Y$ is judging whether the output $G(x,y)$ (which is supposed to be a face image with identity of $x$ and make-up style of  $y$) and the style reference $y$ is in the same style domain, and $D_X$ does the same thing for style domain of $x$.

\textbf{Purifier \textit{$H$}.} In our method, we creatively apply a purifier network $H$ in the training pipeline to ensure the cycle reconstruction measure function well. Cycle reconstruction and cycle consistency loss~\cite{DBLP:conf/iccv/ZhuPIE17} are crucial elements in the unsupervised training process of image-to-image translation tasks. This cycle consistency requirement enforces the generator to learn the mappings between the source and target domain without supervised training data (\textit{e.g.} transferred images for style-transfer task). Generally, cycle consistency loss is defined as $\parallel G(G(x,y),x)  -x\parallel_1$, which measures the distance between reconstruction output and source image. However, in our method, $G$ is supposed to generate adversarial examples which can affect the feature extracting of DNNs, and this characteristic will have a negative influence on the reconstruction path (see our ablation study Fig.~\ref{}) where the adversarial output $G(x,y)$ becomes the input image conversely.

Recently, it is shown that the encoder-decoder models can be used to alleviate the toxicity of adversarial examples or disentangle the adversarial information from them~\cite{,DBLP:conf/cvpr/NaseerKHKP20}. Inspired by these studies, we design a purifier network $H$ with an encoder-decoder architecture. $H$ is supposed to generate the purified images $H(G(x,y))$ with the same content, style, and dimensions as adversarial input images $G(x,y)$ without the adversarial toxicity. 

The purifier $H$ will share the same training process of the main networks $G$ and $D$ and ensure the cycle consistency loss function well. Our experiments show that the existence of $H$ can encourage $G$ to generate adversarial examples with high visual quality and realistic cosmetic style. 

\textbf{Meta-learning Model Zoo \textit{$M$}.} The meta-learning model zoo \textit{$M$} consists of \textit{$K$} pre-trained face recognition models, which have high accuracy on public face images datasets. These local models serve as white-box models when we train our GANs and try to imitate the decision boundaries of potential target models which we cannot access. 

\textcolor{magenta}{Generally, in the conventional way of enhancing the transferability of adversarial examples in a black-box setting, some adversaries will use ensemble training scheme~\cite{DBLP:conf/cvpr/DongLPS0HL18}, which means \iffalse every model in the local model zoo offers the adversarial loss mentioned in Eq.~\ref{eq:adversarial fomulation} and these results will be calculated to find the common gradient of black-box adversarial attacks\fi multiple local models are used to compose a substitute model to imitate the decision boundaries of potential target models. This measure improves the transferability of adversarial examples compared to white-box attack algorithms, as it tries to avoid the over-fitting on certain single white-box model. Recently, the meta-learning method~\cite{DBLP:journals/corr/abs-2004-05439} is considered superior to ensemble training due to its excellent performance in XXX. Some studies~\cite{DBLP:journals/corr/abs-2108-04204,DBLP:conf/ijcai/YinWYGKDLL21} have shown the promising future of it in the black-box attacks. In this paper, we use the similar meta-learning pipeline mentioned in~\cite{DBLP:conf/ijcai/YinWYGKDLL21}.} \textit{Reconsider needed}

This module can be regarded as a large white-box model to easily understand. The detailed pipeline of meta-learning will be introduced later. 


% \textbf{Auxiliary Model \textit{$F$}.}
% \subsection{Training Phases}

\textcolor{magenta}{\subsection{Objective Function}} 
% 这些公式下标可能有问题，G和H是否会同时出现？问一下张老师
\textbf{GAN Loss.} We encourage \textit{$D_X$} and \textit{$D_Y$} to distinguish whether an input is real or gerenrated by $G$ for source domain $X$ and reference domain $Y$ respectively, while $G$ tries to generate realistic images to deceive \textit{$D_X$} and \textit{$D_Y$}. For $H$, we encourage it to reconstruct the real performance of $G$ in style transfer. So the GAN objective can be formulated as follows:

\begin{equation}\label{eq:LossGAN_D}
\begin{aligned}
    L^{GAN}_D =&- \mathbb{E}_{x\thicksim P_X}[logD_X(x)] - \mathbb{E}_{y\thicksim P_Y}[logD_Y(y)]\\&- \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[log(1-D_X(G(y,x)))]
    \\&- \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[log(1-D_Y(G(x,y)))], 
    % \\&- \mathbb{E}_{x\thicksim P_X,y\thicksim P_X}[log(1-D_X(H(G(y,x))))] 
    % \\&- \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[log(1-D_Y(H(G(x,y))))]
\end{aligned}
\end{equation}
\begin{equation}\label{eq:LossGAN_G}
\begin{aligned}
    L^{GAN}_G =&- \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[log(D_X(G(y,x)))]
    \\&- \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[log(D_Y(G(x,y)))],
\end{aligned}
\end{equation}
\begin{equation}\label{eq:LossGAN_H}
\begin{aligned}
    L^{GAN}_H =&- \mathbb{E}_{x\thicksim P_X,y\thicksim P_X}[log(D_X(H(G(y,x))))] 
    \\&- \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[log(D_Y(H(G(x,y))))].
\end{aligned}
\end{equation}

\textbf{Cycle consistency loss.} The cycle consistency constraint~\cite{DBLP:conf/iccv/ZhuPIE17} plays a crucial role in the unsupervised training process of image-to-image translation GANs. In our method, the generator $G$ turns clean images into adversarial examples. so we use additional nets $H$ to ensure the cycle consistency loss function normally. The cycle consistency loss is calculated by:
\begin{equation}\label{eq:LossCycle}
\begin{aligned}
    L^{rec}_G &= \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[\parallel G(H(G(x,y)),x)  -x\parallel_1]
    \\&+ \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[\parallel G(H(G(y,x)),y)  -y\parallel_1].
\end{aligned}
\end{equation}
Note that we don't input the cycle reconstruction result(i.e. $G(H(G(x,y)),x)$) into $H$ again because we also encourage the adversarial examples generated by $G$ to look as similar as possible to clean images.

\textbf{Makeup loss.} The histogram matching~\cite{DBLP:conf/mm/LiQDLYZL18} which denotes as $HM(x,y)$ is used to simulate the color distribution of reference $y$ while preserves the content information of $x$. Here, we use this objective function to ensure the make-up similarity on lips, eye shadows, and face regions as well as reconstruction ability of $H$. The makeup loss is defined as:
\begin{equation}\label{eq:LossMakeup_G}
\begin{aligned}
    L^{makeup}_G &= \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[\parallel G(x,y) - HW(x,y) \parallel_2]\\&+ \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[\parallel G(y,x) - HW(y,x) \parallel_2],
\end{aligned}
\end{equation}
\begin{equation}\label{eq:LossMakeup_H}
\begin{aligned}
    L^{makeup}_H &= \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[\parallel H(G(x,y)) - HW(x,y) \parallel_2]\\&+ \mathbb{E}_{x\thicksim P_X,y\thicksim P_Y}[\parallel H(G(y,x)) - HW(y,x) \parallel_2].
\end{aligned}
\end{equation}

\textbf{Adversarial attack loss.} The adversarial loss is usually a distance function which measures the similarity  of two outputs given by DNN models. For impersonating (target) attack on face recognition models, the adversarial loss can be defined as: $L_{target} = 1 - cos[M_k(z),M_k(x)]$, where $M_k$ represents a local feature extractor pre-trained on face images datasets, and cosine similarity~\cite{} is used as distance function.

In this paper, we use a meta-learning scheme in our framework to gain adversarial examples with good transferability. Specifically, $K-1 $ models are randomly selected from the meta-learning model zoo $M$ in each iteration to serve as the feature extractors mentioned above. We use $\{M^{train}_k\}_{k=1,...,K-1}$ to represent these models and $M_K$ to represent the remaining model. Taking the training process of $G$ for example, we divide every iteration into two parts: the meta-training phase and the meta-testing phase. In the meta-training phase, the $k$-th model $M^{train}_k \in \{M^{train}_k\}_{k=1,...,K-1}$ is the feature extractor, gives the feature maps of the images with target identification $z$ and the out image of $G$ to calculate the adversarial loss. Then, we update $G$ by this loss function added with other functions mentioned above and get $G^k_{temp}$. Next, in the meta-training phase, we choose $M_K$ as the feature extractor and feed it with $z$ and the output of $G^k_{temp}$, and update $G^k_{temp}$ to $G_k$ with loss given by $M_K$ (here we only consider adversarial loss). So, there are $K-1$ pairs of meta-training phase and meta-testing phase in every iteration. At the end of each iteration, we update $G$ by $G=\frac{1}{K-1}\sum^{K-1}_{k=1}G_k$. The adversarial attack losses of $G$ are as follows:
\begin{equation}\label{eq:LossAdvG_meta-train}
\begin{aligned}
    L^{meta-train}_G =&2 - cos[M^{trian}_k(z),M^{trian}_k(G(x,y))] \\
    &- cos[M^{trian}_k(z),M^{trian}_k(G(y,x))],
\end{aligned}
\end{equation}

\begin{equation}\label{eq:LossAdvG_meta-test}
\begin{aligned}
    L^{meta-test}_G =&2 - cos[M_K(z),M_K(G(x,y))] \\
    &- cos[M_K(z),M_K(G(y,x))].
\end{aligned}
\end{equation}

For the purifier $H$, the training goal is to let $H$ have ability to alleviate the toxicity of outputs from $G$. So the adversarial attack losses of $H$ are defined as: 
\begin{equation}\label{eq:LossAdvH_meta-train}
\begin{aligned}
    L^{meta-train}_H =&2 - cos[M^{trian}_k(x),M^{trian}_k(H(G(x,y)))] \\
    &- cos[M^{trian}_k(y),M^{trian}_k(H(G(y,x)))],
\end{aligned}
\end{equation}

\begin{equation}\label{eq:LossAdvH_meta-test}
\begin{aligned}
    L^{meta-test}_H =&2 - cos[M_K(x),M_K(H(G(x,y)))] \\
    &- cos[M_K(y),M_K(H(G(y,x)))].
\end{aligned}
\end{equation}
% \textbf{Perceptual loss.}

\textbf{Total loss.} The total loss for $D_X$ and $D_Y$ is as follows:
\begin{equation}\label{eq:LossD}
\begin{aligned}
    L_D = \lambda_{GAN}L^{GAN}_D,
\end{aligned}
\end{equation}
The total loss of $G$ in meta-training phase is defined as:
\begin{equation}\label{eq:LossG_mtr}
\begin{aligned}
    L^{mtr}_G &= \lambda_{GAN}L^{GAN}_G + \lambda_{cyc}L^{rec}_G \\
    &+ \lambda_{make}L^{makeup}_G +\lambda_{adv}L^{meta-train}_G,
\end{aligned}
\end{equation}
The total loss of $G$ in meta-testing phase is defined as:
\begin{equation}\label{eq:LossG_mte}
\begin{aligned}
    L^{mte}_G &= \lambda_{adv}L^{meta-test}_G,
\end{aligned}
\end{equation}
The total loss of $H$ in meta-training phase is defined as:
\begin{equation}\label{eq:LossH_mtr}
\begin{aligned}
    L^{mtr}_H &= \lambda^H_{GAN}L^{GAN}_H + \lambda_{make}L^{makeup}_H
    + \lambda_{adv}L^{meta-train}_H,
\end{aligned}
\end{equation}
The total loss of $H$ in meta-testing phase is defined as:
\begin{equation}\label{eq:LossH_mte}
\begin{aligned}
    L^{mte}_H &= \lambda_{adv}L^{meta-test}_H,
\end{aligned}
\end{equation}
Where hyper-parameters $\lambda_{GAN},\lambda^H_{GAN},\lambda_{cyc},\lambda_{make},\lambda_{adv}$ is used to balance the different objectives. The training process is illustrated in Alg.~\ref{alg}.
\input{section/algorithm}

